KPEval: Towards Fine-Grained Semantic-Based Keyphrase Evaluation

Despite the significant advancements in keyphrase extraction and keyphrase generation methods, the predominant approach for evaluation mainly relies on exact matching with human references. This scheme fails to recognize systems that generate keyphrases semantically equivalent to the references or diverse keyphrases that carry practical utility. To better assess the capability of keyphrase systems, we propose KPEval, a comprehensive evaluation framework consisting of four critical aspects: reference agreement, faithfulness, diversity, and utility. For each aspect, we design semantic-based metrics to reflect the evaluation objectives. Meta-evaluation studies demonstrate that our evaluation strategy correlates better with human preferences compared to a range of previously proposed metrics. Using KPEval, we re-evaluate 23 keyphrase systems and discover that (1) established model comparison results have blind-spots especially when considering reference-free evaluation; (2) large language models are underestimated by prior evaluation works; and (3) there is no single best model that can excel in all the aspects.

==> tables/all_results_ref_based.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c c c c | c c c c }
 \hline
 \multirow{3}{*}{\textbf{ID}}  & \multirow{3}{*}{\textbf{Model}}  & \multicolumn{4}{c|}{\textbf{KP20k}} & \multicolumn{4}{c}{\textbf{KPTimes}} \\
  &  & \multicolumn{1}{c}{\textbf{Sal.}} & \multicolumn{1}{c}{\textbf{Cov.}} &\multicolumn{1}{c}{\textbf{Sal.+Cov.}} & \multicolumn{1}{c|}{\textbf{Cov.}} & \multicolumn{1}{c}{\textbf{Sal.}} & \multicolumn{1}{c}{\textbf{Cov.}} &\multicolumn{1}{c}{\textbf{Sal.+Cov.}} & \multicolumn{1}{c}{\textbf{Cov.}} \\
  & & $SemP\uparrow$ & $SemR\uparrow$ & $SemF1\uparrow$ & $SemCov\uparrow$ & $SemP\uparrow$ & $SemR\uparrow$ & $SemF1\uparrow$ & $SemCov\uparrow$ \\
 \hline
\textbf{M1} & TF-IDF & 0.431 & 0.524 & 0.463 & 0.814 & 0.403 & 0.557 & 0.461 & 0.802 \\
\textbf{M2} & TextRank & 0.432 & 0.518 & 0.460 & 0.813 & 0.457 & 0.532 & 0.483 & 0.800 \\
\textbf{M3} & MultipartiteRank & 0.364 & 0.548 & 0.429 & 0.814 & 0.410 & 0.575 & 0.472 & 0.806 \\
\textbf{M4} & Kea & 0.452 & 0.533 & 0.479 & 0.816 & 0.427 & 0.575 & 0.484 & 0.806 \\
\textbf{M5} & BERT+CRF & \underline{\textbf{0.675}} & 0.447 & 0.515 & 0.606 & 0.741 & 0.459 & 0.550 & 0.542 \\
\textbf{M6} & HyperMatch & 0.505 & \underline{\textbf{0.631}} & 0.549 & 0.756 & 0.493 & 0.655 & 0.554 & 0.757 \\
\textbf{M7} & CatSeq &\textbf{0.596} & 0.531 & 0.548 & 0.791 & 0.723 & 0.714 & 0.708 & 0.856 \\
\textbf{M8} & CatSeqTG-2RF1 & 0.550 & 0.579 & 0.553 & 0.824 & n/a   & n/a   & n/a   & n/a   \\
\textbf{M9} & ExHiRD-h & 0.587 & 0.559 & 0.562 & 0.814 & 0.725 & 0.713 & 0.709 & 0.858 \\
\textbf{M10} & SEG-Net & 0.560 & 0.596 & 0.565 & 0.826 & n/a & n/a & n/a & n/a \\
\textbf{M11} & Transformer & 0.558 & 0.593 & 0.562 & 0.823 & 0.720 & 0.736 & 0.717 & 0.864 \\
\textbf{M12} & SetTrans & 0.570 & \textbf{0.623} & \textbf{0.583} & \underline{\textbf{0.835}} & 0.662 & \textbf{0.801} & 0.716 & 0.871 \\
\textbf{M13} & SciBERT-G & 0.587 & 0.590 & \textbf{0.577} & 0.823 & \underline{\textbf{0.784}} & 0.737 & 0.749 & 0.868 \\
\textbf{M14} & BART-large  & 0.567 & 0.607 & 0.574 & \textbf{0.828} & \textbf{0.768} & \textbf{0.796} & \underline{\textbf{0.770}} & \underline{\textbf{0.885}} \\
\textbf{M15} & KeyBART & 0.580 & 0.599 & \textbf{0.577} & 0.824 & 0.751 & \underline{\textbf{0.807}} & \textbf{0.766} & \underline{\textbf{0.885}} \\
\textbf{M16} & SciBART-large+OAGKX & \textbf{0.601} & \textbf{0.623} & \underline{\textbf{0.601}} & \underline{\textbf{0.835}} & \textbf{0.782} & 0.766 & \textbf{0.763} & \textbf{0.879} \\
\textbf{M17} & text-davinci-003 (0-shot) & 0.433 & 0.616 & 0.498 & 0.826 & 0.383 & 0.620 & 0.467 & 0.809 \\
\textbf{M18} & text-davinci-003 (5-shot) & 0.503 & 0.599 & 0.535 & 0.825 & 0.549 & 0.643 & 0.582 & 0.824 \\
\textbf{M19} & Amazon Comprehend & 0.224 & 0.324 & 0.259 & 0.765& 0.258 & 0.347 & 0.292 & 0.761 \\
\textbf{M20} & Azure Cognitive Services & 0.387 & 0.536 & 0.440 & 0.813 & 0.312 & 0.425 & 0.355 & 0.782 \\
 \hline
 \end{tabular}
 }
 % \vspace{-2mm}
\caption{Reference-based evaluation results. The best result is underlined and the top three results are boldfaced. } 
 \label{tab:all-results-ref-based}
 % \vspace{-3mm}
 
\end{table*}

==> tables/all_results_ref_free.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c | c c c c c c c c}
 \hline
 \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#KP}} & \multicolumn{2}{c}{\textbf{Naturalness}} & \multicolumn{2}{c}{\textbf{Faithfulness}} & \multicolumn{2}{c}{\textbf{Diversity}} & \multicolumn{2}{c}{\textbf{Utility}} \\
& & & $U \uparrow$& $G \uparrow$ & $U \uparrow$ & $G \uparrow$& $dup\downarrow$ &$emb\_sim\downarrow$ & $RR@5\uparrow$ & $Spare_5@5\uparrow$ \\
 \hline
 \textbf{M0} & Human References & 5.3 & 0.833 & 4.26 & 0.697 & 3.86 & \underline{\textbf{0.073}} & 0.133 & 0.698 & 0.500 \\
\textbf{M1} & TF-IDF & 10.0 & 0.610 & 3.76 & 0.696 & 4.52 & 0.396 & 0.161 & 0.848 & 0.393 \\
\textbf{M2} & TextRank & 10.0 & 0.761 & 3.76 & 0.737 & 4.57 & 0.391 & 0.180 & 0.877 & 0.416 \\
\textbf{M3} & MultipartiteRank & 10.0 & 0.742 & 3.77 & 0.712 & 4.35 & 0.148 & \textbf{0.092} & 0.922 & 0.472 \\
\textbf{M4} & Kea & 10.0 & 0.611 & 3.76 & 0.715 & 4.51 & 0.445 & 0.175 & 0.861 & 0.388 \\
\textbf{M5} & BERT+CRF & 3.6 & 0.762 & 4.05 & \underline{\textbf{0.801}} & \textbf{4.63} & 0.137 & 0.399 & 0.633 & 0.487 \\
\textbf{M6} & HyperMatch & 10.0 & 0.708 & 3.45 & 0.772 & 4.14 & 0.297 & 0.233 & 0.854 & 0.496 \\
\textbf{M7} & CatSeq & 7.2 & 0.837 & 4.27 & 0.774 & 4.51 & 0.370 & 0.310 & 0.809 & 0.571 \\
\textbf{M8} & CatSeqTF+2RF1 & 7.9 & \underline{\textbf{0.872}} & \underline{\textbf{4.47}} & 0.734 & 3.98 & 0.355 & 0.251 & 0.795 & \textbf{0.613} \\
\textbf{M9} & ExHiRD-h & 5.5 & 0.851 & 4.31 & \textbf{0.781} & 4.50 & 0.214 & 0.195 & 0.880 & 0.576 \\
\textbf{M10} & SEG-Net & 11.0 & 0.793 & 3.88 & 0.757 & 4.50 & 0.260 & 0.177 & 0.922 & 0.587 \\
\textbf{M11} & Transformer & 8.2 & 0.837 & \textbf{4.32} & 0.747 & 4.37 & 0.289 & 0.239 & 0.863 & 0.587 \\
\textbf{M12} & SetTrans & 7.7 & \textbf{0.855} & \textbf{4.33} & 0.766 & 4.38 & 0.308 & 0.203 & 0.909 & 0.541 \\
\textbf{M13} & SciBERT-G & 6.1 & 0.841 & 4.28 & 0.762 & 4.40 & 0.152 & 0.177 & 0.848 & 0.579 \\
\textbf{M14} & BART-large & 6.6 & 0.847 & 4.23 & 0.759 & 4.25 & 0.144 & 0.168 & 0.872 & 0.568 \\
\textbf{M15} & KeyBART & 6.0 & 0.849 & 4.27 & 0.765 & 4.32 & 0.130 & 0.163 & 0.864 & 0.568 \\
\textbf{M16} & SciBART-large+OAGKX & 6.1 & 0.846 & 4.29 & 0.766 & 4.44 & \textbf{0.129} & 0.158 & 0.871 & 0.571 \\
\textbf{M17} & text-davinci-003 (0-shot) & 9.5 & 0.838 & 4.08 & 0.777 & \textbf{4.72} & 0.143 & 0.110 & \underline{\textbf{0.979}} & \textbf{0.599} \\
\textbf{M18} & text-davinci-003 (5-shot) & 6.5 & \textbf{0.857} & 4.21 & \textbf{0.790} & \underline{\textbf{4.74}} & \textbf{0.084} & 0.113 & \textbf{0.975} & \underline{\textbf{0.630}} \\
\textbf{M19} & Amazon Comprehend & 10.0 & 0.822 & 3.25 & 0.693 & 3.91 & 0.436 & \textbf{0.103} & 0.565 & 0.254 \\
\textbf{M20} & Azure Cognitive Services & 10.0 & 0.818 & 3.77 & 0.778 & 4.53 & 0.198 & \underline{\textbf{0.068}} & \textbf{0.955} & 0.552 \\
 \hline
 \end{tabular}
 }
 % \vspace{-2mm}
 \caption{Reference-free evaluation results on KP20k for all the benchmarked models. The best result is underlined and the top three results are boldfaced. $U$ = UniEval, $G$ = ChatGPT, $dup$ = $dup\_token\_ratio$. Due to cost constraints, the scores reported in $G$ columns are measured with the first 500 documents. } 
 \label{tab:all-results-ref-free-kp20k}
 % \vspace{-3mm}
 
\end{table*}


\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c | c c c c c c c c}
 \hline
 \multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#KP}} & \multicolumn{2}{c}{\textbf{Naturalness}} & \multicolumn{2}{c}{\textbf{Faithfulness}} & \multicolumn{2}{c}{\textbf{Diversity}} & \multicolumn{2}{c}{\textbf{Utility}} \\
& & & $U \uparrow$& $G \uparrow$ & $U \uparrow$ & $G \uparrow$& $dup\downarrow$ &$emb\_sim\downarrow$ & $RR@5\uparrow$ & $Spare_5@5\uparrow$ \\
 \hline
 \textbf{M0} & Human References & 5.0 & 0.812 & \textbf{4.61} & 0.701 & 3.48 & \textbf{0.069} & 0.203 & 0.515 & 0.420 \\
\textbf{M1} & TF-IDF & 10.0 & 0.616 & 4.11 & 0.658 & 3.98 & 0.175 & 0.163 & 0.798 & 0.406 \\
\textbf{M2} & TextRank & 10.0 & 0.679 & 4.12 & 0.667 & 4.03 & 0.371 & 0.246 & 0.745 & 0.347 \\
\textbf{M3} & MultipartiteRank & 10.0 & 0.693 & 4.18 & 0.670 & \textbf{4.05} & 0.123 & \textbf{0.150} & \textbf{0.837} & 0.437 \\
\textbf{M4} & Kea & 10.0 & 0.615 & 4.10 & 0.699 & \textbf{4.07} & 0.219 & 0.175 & \textbf{0.843} & 0.420 \\
\textbf{M5} & BERT+CRF & 2.3 & 0.704 & 3.98 & \underline{\textbf{0.769}} & 3.90 & 0.072 & 0.556 & 0.402 & 0.372 \\
\textbf{M6} & HyperMatch & 10.0 & 0.695 & 4.24 & 0.703 & 3.68 & 0.124 & 0.271 & 0.679 & 0.320 \\
\textbf{M7} & CatSeq & 5.9 & 0.812 & 4.59 & 0.683 & 3.34 & 0.191 & 0.257 & 0.524 & 0.469 \\
\textbf{M8} & CatSeqTG-2RF1 & n/a & n/a & n/a & n/a & n/a & n/a & n/a & n/a & n/a \\
\textbf{M9} & ExHiRD-h & 5.8 & 0.801 & 4.58 & 0.680 & 3.30 & 0.149 & 0.238 & 0.535 & 0.474 \\
\textbf{M10} & SEG-Net & n/a & n/a & n/a & n/a & n/a & n/a & n/a & n/a & n/a \\
\textbf{M11} & Transformer & 5.7 & 0.803 & 4.60 & 0.658 & 3.10 & 0.133 & 0.231 & 0.522 & 0.474 \\
\textbf{M12} & SetTrans & 8.4 & 0.808 & 4.60 & 0.645 & 3.00 & 0.210 & 0.232 & 0.584 & 0.410 \\
\textbf{M13} & SciBERT-G & 4.5 & 0.812 & 4.60 & 0.716 & 3.51 & 0.064 & 0.208 & 0.594 & 0.473 \\
\textbf{M14} & BART-large & 5.4 & 0.809 & 4.60 & 0.706 & 3.43 & 0.074 & 0.203 & 0.641 & \textbf{0.482} \\
\textbf{M15} & KeyBART & 5.9 & 0.806 & 4.55 & 0.696 & 3.35 & 0.086 & 0.206 & 0.639 & 0.480 \\
\textbf{M16} & SciBART-large+OAGKX & 4.8 & 0.810 & 4.60 & 0.718 & 3.52 & \textbf{0.069} & 0.203 & 0.628 & \textbf{0.482} \\
\textbf{M17} & text-davinci-003 (0-shot) & 14.1 & \textbf{0.840} & \textbf{4.65} & 0.690 & 3.98 & 0.082 & \textbf{0.137} & \underline{\textbf{0.871}} & \underline{\textbf{0.597}} \\
\textbf{M18} & text-davinci-003 (5-shot) & 6.7 & \underline{\textbf{0.859}} & \underline{\textbf{4.78}} & \textbf{0.725} & \underline{\textbf{4.28}} &  \underline{\textbf{0.044}} & 0.188 & 0.829 & \textbf{0.582} \\
\textbf{M19} & Amazon Comprehend & 10.0 & \textbf{0.818} & 3.62 & 0.617 & 3.17 & 0.291 & 0.203 & 0.492 & 0.123 \\
\textbf{M20} & Azure Cognitive Services & 10.0 & 0.769 & 4.09 & \textbf{0.728} & 3.71 & 0.140 & \underline{\textbf{0.133}} & 0.564 & 0.338 \\
 \hline
 \end{tabular}
 }
 % \vspace{-2mm}
 \caption{Reference-free evaluation results on KPTimes for all the benchmarked models. The best result is underlined and the top three results are boldfaced. $U$ = UniEval, $G$ = ChatGPT, $dup$ = $dup\_token\_ratio$. Due to cost constraints, the scores reported in $G$ columns are measured with the first 500 documents. } 
 \label{tab:all-results-ref-free-kptimes}
 % \vspace{-3mm}
 
\end{table*}


==> tables/chatgpt_faithfulness_prompt.tex <==
\begin{figure}[]
    \centering
    \small
    \resizebox{\linewidth}{!}{
    \fbox{\begin{tabular}{ p{1.1\columnwidth} }
    % \hline
   Given a keyphrase with the corresponding document, rate its faithfulness on a scale from 1 to 5 (1 for not faithful at all and 5 for perfectly faithful). If a keyphrase is irrelevant, i.e., not actually discussed by the document, then it should receive a low faithfulness score. Abbreviations may be treated as faithful phrases as long as they are valid. [digit] symbols may also be treated as faithful. Note that phrases appear as a subtring of the text can be an unfaithful keyphrase, and that phrases absent from the text can be perfectly faithful. You may use partial scores (decimals). Only output score. Do not output anything else. \\ \\

    Document: security personalization for internet and web services . [sep] the growth of the internet has been accompanied by the growth of internet services ( e.g. , e commerce , e health ) . this proliferation of services and the increasing attacks on them by malicious individuals have highlighted the need for service security . the security requirements of an internet or pleb service may be specified in a security policy . the provider of the service is then responsible. , for implementing the security measures contained in the policy . \\ \\
    
    Keyphrase: security personalization \\
    Faithfulness: 5 \\
    Keyphrase: cyberattacks \\
    Faithfulness: 5 \\
    Keyphrase: internet \\
    Faithfulness: 4 \\
    Keyphrase: security model \\
    Faithfulness: 3 \\
    Keyphrase: customer service \\
    Faithfulness: 2 \\
    Keyphrase: public policy \\
    Faithfulness: 2 \\
    Keyphrase: infrastructure \\
    Faithfulness: 2 \\
    
    Document: X \\
    Keyphrase: p\_i \\
    Faithfulness: \\
    % \hline
    \end{tabular}}}
    % \vspace{-2mm}
    \caption{Prompts used for instructing ChatGPT to evaluation the faithfulness of a keyphrase.}
    % \vspace{-1mm}
    \label{chatgpt-faithfulness-prompt}
    % \vspace{-4mm}
\end{figure}


==> tables/human_eval_results.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c c c c | c c c c }
 \hline
\multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{KP20k}} & \multicolumn{4}{c}{\textbf{KPTimes}} \\
 & & \multicolumn{1}{c}{\textbf{Sal. $\uparrow$}} & \multicolumn{1}{c}{\textbf{Cov. $\uparrow$}} &\multicolumn{1}{c}{\textbf{Sal.+Cov. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$} & \multicolumn{1}{c}{\textbf{Sal. $\uparrow$}} & \multicolumn{1}{c}{\textbf{Cov. $\uparrow$}} & \multicolumn{1}{c}{\textbf{Sal.+Cov. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$}\\
 \hline
\textbf{M3} & MultipartiteRank & 0.447 & 0.434 & 0.436 & 3.98 & 0.512 & 0.492 & 0.494 & 4.48 \\
\textbf{M7} & CatSeq & \textbf{0.601} & 0.518 & 0.550 & 2.80 & 0.735 & 0.700 & 0.709 & 2.50 \\
\textbf{M12} & SetTrans & 0.575 & 0.589 & \textbf{0.571} & \textbf{2.46} & 0.666 & \textbf{0.804} & 0.722 & 2.24 \\
\textbf{M15} & KeyBART & - & - & - & - & \textbf{0.741} & 0.796 & \textbf{0.759} & \textbf{2.00} \\
\textbf{M16} & SciBART-large+OAGKX & 0.568 & 0.590 & 0.570 & 2.54 & - & - & - & - \\
\textbf{M18} & text-davinci-003 (5-shot) & 0.493 & \textbf{0.601} & 0.535 & 3.22 & 0.565 & 0.638 & 0.593 & 3.78 \\
 \hline
 \end{tabular}
 }
 % \vspace{-2mm}
 \caption{Human evaluation results. For M3, we only use its top 5 predictions for consistency with other systems. "Avg. Rank" is the averaged rank over five systems using the F1 score calculated from human annotations. The raw Likert scores are rescaled to the range [0, 1] and then used to calculate the precision, recall, and F1.}
 \label{tab:human-eval-results}
 % \vspace{-3mm}
 
\end{table*}


\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c c c c | c c c c }
 \hline
\multirow{2}{*}{\textbf{ID}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c|}{\textbf{KP20k}} & \multicolumn{4}{c}{\textbf{KPTimes}} \\
 & & \multicolumn{1}{c}{\textbf{Nat. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$} & \multicolumn{1}{c}{\textbf{Faith. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$} & \multicolumn{1}{c}{\textbf{Nat. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$} & \multicolumn{1}{c}{\textbf{Faith. $\uparrow$}} & \textbf{Avg. Rank $\downarrow$}  \\
 \hline
\textbf{M0} & Human References & 3.94 & 3.16 & 4.02 & 3.82 & 4.07 & 2.68 & 4.12 & 2.62 \\
\textbf{M3} & MultipartiteRank & 3.88 & 3.54 & 4.56 & 2.02 & 3.63 & 4.32 & 4.48 & \textbf{1.48} \\
\textbf{M7} & CatSeq & 4.07 & 2.10 & 4.47 & 2.34 & 4.13 & 1.96 & 4.05 & 3.00 \\
\textbf{M12} & SetTrans & 4.14 & 2.06 & 4.43 & 3.02 & 4.16 & 2.16 & 3.86 & 3.64 \\
\textbf{M15} & KeyBART & - & - & - & - & 4.08 & 2.32 & 4.11 & 2.76 \\
\textbf{M16} & SciBART-large+OAGKX & 4.07 & 2.30 & 4.43 & 2.54 & - & - & - & - \\
\textbf{M18} & text-davinci-003 (5-shot) & \textbf{4.16} & \textbf{1.84} & \textbf{4.64} & \textbf{1.26} & \textbf{4.20} & \textbf{1.56} & \textbf{4.45} & 1.50 \\
 \hline
 \end{tabular}
 }
 % \vspace{-2mm}
 \caption{Human evaluation results. For M3, we only use its top 5 predictions for consistency with other systems. "Avg. Rank" is the averaged rank over five systems using the F1 score calculated from human annotations.}
 \label{tab:human-eval-results-ref-free}
 % \vspace{-3mm}
 
\end{table*}

==> tables/meta_eval_matching_strategy.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table}[]
    \centering
    % \resizebox{\columnwidth}{!}{%
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l | c c c | c c c  }
    \hline
    &   \multicolumn{3}{c|}{\textbf{KP20k}} & \multicolumn{3}{c}{\textbf{KPTimes}} \\
    & $r$ & $\rho$ & $\tau$ & $r$ & $\rho$ & $\tau$ \\
    \hline
    Exact Matching & 0.705 & 0.689 & 0.590 & 0.768 & 0.792 & 0.684 \\
    Substring Matching & 0.749 & 0.735 & 0.629 & 0.787 & 0.788 & 0.681 \\
    BertScore Precision & 0.562 & 0.597 & 0.436 & 0.694 & 0.729 & 0.553 \\
    Semantic Matching  & \textbf{0.898} & \textbf{0.884} & \textbf{0.735} & \textbf{0.926} & \textbf{0.925} & \textbf{0.794} \\
    \hline
    \end{tabular}
    }
    % \vspace{-2mm}
    \caption{Correlation between phrase-level decision of humans and various matching strategies. Semantic matching leads other strategies by a large margin.}
    \label{tab:meta-eval-matching}
    % \vspace{-3mm}
    
\end{table}



==> tables/metric_bias.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 % \resizebox{\columnwidth}{!}{%
 \resizebox{\linewidth}{!}{
 \begin{tabular}{l | c | c c c c c c c c | c c c c c c c c }
 \hline
\multirow{3}{*}{\textbf{ID}} & \multirow{3}{*}{\textbf{Model}} & \multicolumn{8}{c|}{\textbf{KP20k}} & \multicolumn{8}{c}{\textbf{KPTimes}} \\
 & & \multicolumn{4}{c}{\textbf{UniEval}} & \multicolumn{4}{c|}{\textbf{ChatGPT}} & \multicolumn{4}{c}{\textbf{UniEval}} & \multicolumn{4}{c}{\textbf{ChatGPT}} \\
 & & \textbf{H $\uparrow$} & \textbf{Tie} & \textbf{M $\uparrow$} & $\frac{M}{H}$ & \textbf{H $\uparrow$} & \textbf{Tie} & \textbf{M $\uparrow$} & $\frac{M}{H}$ & \textbf{H $\uparrow$} & \textbf{Tie} & \textbf{M $\uparrow$} & $\frac{M}{H}$ & \textbf{H $\uparrow$} & \textbf{Tie} & \textbf{M $\uparrow$} & $\frac{M}{H}$ \\
 \hline
 \multicolumn{10}{l}{\textbf{\textit{Naturalness}}}  \\
 \hdashline
 \textbf{M0} & Human & 12 & 64 & 24 & \textbf{1.93} & 13 & 61 & 27 & \textbf{2.09} & 9 & 69 & 22 & 2.45 & 4 & 63 & 33 & 8.10 \\
 \textbf{M3} & MultipartiteRank & 16 & 66 & 18 & 1.10 & 20 & 65 & 15 & 0.73 & 13 & 59 & 28 & 2.19 & 4 & 59 & 36 & 8.27 \\
 \textbf{M7} & CatSeq & 11 & 76 & 13 & 1.26 & 16 & 67 & 17 & 1.04 & 10 & 71 & 17 & 1.71 & 2 & 70 & 28 & 14.00 \\
 \textbf{M12} & SetTrans & 8 & 77 & 14 & 1.73 & 13 & 68 & 19 & 1.52 & 10 & 74 & 16 & 1.54 & 4 & 68 & 29 & 7.65 \\
 \textbf{M15} & KeyBART & - & - & - & - & - & - & - & - & 10 & 72 & 18 & 1.79 & 5 & 64 & 31 & 5.90 \\
 \textbf{M16} & SciBART-large+OAGKX & 8 & 76 & 15 & 1.83 & 13 & 65 & 22 & 1.66 & - & - & - & - & - & - & - & - \\
 \textbf{M18} & text-davinci-003 (5-shot) & 10 & 78 & 11 & 1.09 & 19 & 65 & 17 & 0.90 & 3 & 79 & 17 & \textbf{5.00} & 2 & 65 & 34 & \textbf{21.40} \\
 \hline
 \multicolumn{10}{l}{\textbf{\textit{Faithfulness}}} \\
 \hdashline
 \textbf{M0} & Human & 11 & 76 & 12 & \textbf{1.09} & 19 & 63 & 17 & 0.92 & 18 & 73 & 9 & 0.48 & 41 & 49 & 9 & 0.22 \\
 \textbf{M3} & MultipartiteRank & 20 & 79 & 2 & 1.07 & 11 & 79 & 10 & 0.89 & 30 & 67 & 3 & 0.09 & 17 & 72 & 12 & \textbf{0.69} \\
 \textbf{M7} & CatSeq & 10 & 82 & 8 & 0.79 & 10 & 79 & 10 & 0.97 & 18 & 74 & 7 & 0.39 & 44 & 48 & 8 & 0.19\\
 \textbf{M12} & SetTrans & 8 & 84 & 7 & 0.90 & 10 & 76 & 14 & 1.42 & 20 & 70 & 10 & 0.48 & 45 & 46 & 9 & 0.20 \\
 \textbf{M15} & KeyBART & - & - & - & - & - & - & - & - & 18 & 72 & 9 & \textbf{0.52} & 42 & 50 & 8 & 0.20\\
 \textbf{M16} & SciBART-large+OAGKX & 14 & 80 & 6 & 0.39 & 13 & 76 & 11 & 0.89 & - & - & - & - & - & - & - & - \\
 \textbf{M18} & text-davinci-003 (5-shot) & 13 & 84 & 3 & 0.27 & 7 & 83 & 10 & \textbf{1.45} & 17 & 75 & 7 & 0.42 & 24 & 65 & 12 & 0.49 \\
 \hline
 \end{tabular}
     }
 % \vspace{-2mm}
 \caption{Results on metric bias. We compare the predictions by UniEval/ChatGPT with human annotations. "H$\uparrow$" = percentage where human score is higher. "M$\uparrow$" = percentage where model score is higher. "Tie" = percentage where human score is similar to model predictions.}
 \label{tab:metric-bias}
 % \vspace{-3mm}
 
\end{table*}

==> tables/model_descriptions.tex <==
\setlength{\tabcolsep}{3.5pt}
\begin{table*}[]
 \centering
 \resizebox{0.9\linewidth}{!}{
 \begin{tabular}{l | c | c | c | c | c }
 \hline
 \textbf{ID} & \textbf{Model Name} & \textbf{Reference} & \textbf{Task} & \textbf{Supervised?} &\textbf{Other Properties}  \\
 \hline
\textbf{M1} & TF-IDF & \citet{tf-idf} & KPE & No & statistical KPE \\
\textbf{M2} & TextRank &  \citet{mihalcea-tarau-2004-textrank} & KPE & No & graph-based KPE \\
\textbf{M3} & MultipartiteRank & \citet{boudin-2018-unsupervised} & KPE & No & graph-based KPE \\
\textbf{M4} & Kea & \citet{witten1999kea} & KPE & Yes & feature-based KPE \\
\textbf{M5} & BERT+CRF & \citet{2212.10233} & KPE & Yes & PLM \\
\textbf{M6} & HyperMatch & \citet{song-etal-2022-hyperbolic} & KPE & Yes & PLM \\
\textbf{M7} & CatSeq & \citet{yuan-etal-2020-one} & KPG & Yes & One2Seq \\
\textbf{M8} & CatSeqTG-2RF1 & \citet{chan-etal-2019-neural} & KPG & Yes & RL, One2Seq \\
\textbf{M9} & ExHiRD-h & \citet{chen-etal-2020-exclusive} & KPG & Yes & One2Seq \\
\textbf{M10} & SEG-Net & \citet{ahmad-etal-2021-select} & KPG & Yes & PLM, KPG \\
\textbf{M11} & Transformer & \citet{ye-etal-2021-one2set} & KPG & 
Yes & One2Seq \\
\textbf{M12} & SetTrans & \citet{ye-etal-2021-one2set} & KPG & Yes & One2Set \\
\textbf{M13} & SciBERT-G & \citet{2212.10233} & KPG & Yes & PLM, One2Seq \\
\textbf{M14} & BART-large & \citet{2212.10233} & KPG & Yes & PLM, One2Seq \\
\textbf{M15} & KeyBART & \citet{kulkarni-etal-2022-learning} & KPG & Yes & PLM+TAPT, One2Seq \\
\textbf{M16} & SciBART-large+OAGKX & \citet{2212.10233} & KPG & Yes & PLM+TAPT, One2Seq \\
\textbf{M17} & text-davinci-003 (0-shot) & - & KPG & No & PLM\\
\textbf{M18} & text-davinci-003 (5-shot) & - & KPG & Yes (few-shot) & in-context learning, PLM \\
\textbf{M19} & Amazon Comprehend & - & KPE & No & blackbox KPE \\
\textbf{M20} & Azure Cognitive Services & - & KPE & No & blackbox KPE \\
 \hline
 \end{tabular}
 }
 \caption{Descriptions of the studied models. "KPE" = "Keyphrase Extraction". "KPG" = "Keyphrase Generation". "PLM" = "Pre-trained Language Model". "TAPT" = "Task-adaptive Pre-training".}
 \label{tab:model-descriptions}
\end{table*}
